An Analytical Framework for mmWave-Enabled V2X Caching

Autonomous vehicles will rely heavily on vehicle-to-everything (V2X) communications to obtain a large amount of information required for navigation and road safety purposes. This can be achieved through: (i) leveraging millimeter-wave (mmWave) frequencies to achieve multi- Gbps data rates, and (ii) exploiting the temporal and spatial correlation of vehicular contents to offload a portion of the traffic from the infrastructure via caching. Characterizing such a system under mmWave directional beamforming, high vehicular mobility, channel fluctuations, and different caching strategies is a complex task. In this article, we propose the first stochastic geometry framework for caching in mmWave V2X networks, which is validated via rigorous Monte Carlo simulation. In addition to common parameters considered in stochastic geometry models, our derivations account for caching as well as the speed and the trajectory of the vehicles. Furthermore, our evaluations provide interesting design insights: (i) higher base station/vehicle densities does not necessarily improve caching performance; (ii) although using a narrower beam leads to a higher SINR, it also reduces the connectivity probability; and (iii) V2X caching can be an inexpensive way of compensating some of the unwanted mmWave channel characteristics.

==> figs/relative_speed_d2d.tex <==
% Relative speed for D2D 
	\begin{tikzpicture}[scale=1, >=stealth]		
		\node[inner sep=0pt] (car) at (-2,0) {\includegraphics[width=25pt]{./figs/car.png}};	
		\draw[->, very thick, color=gcolor4] (-2,0) -- (3,0)  node [midway, below, font=\footnotesize, color=black] {};
		\draw[->, ultra thick, black] (-2,0) -- (5mm, 10mm) node [midway, above, font=\footnotesize, color=black] {$v_t, \theta_t$};
		\draw[->, ultra thick, black] (-2,0) -- (-2mm, -8mm) node [midway, below, font=\footnotesize, color=black] {$v_r, \theta_r$};
		\draw [gray, thin] (5mm, 10mm) -- (30mm, 0mm);
		\draw [gray, thin] (-2mm, -8mm) -- (30mm, 0mm);
		\node at (35mm, 0mm) [inner sep=0pt, minimum size=3mm, font=\scriptsize]{$v', \beta$};
	\end{tikzpicture}

